The study of r-process nucleosynthesis in binary neutron star mergers: Nucleonic weak interactions and nuclear uncertainties

A long-standing scientific puzzle has been to explain the origin of the heaviest elements in the Universe and, more particularly, the production of the elements heavier than iron up to uranium. The rapid neutron capture process (or r-process) is known to synthesize about 50\% of these heavy elements and the long-lived actinides observed in our solar system and so-called metal-poor r-process-enhanced stars. This thesis aims to study the r-process nucleosynthesis and some of the uncertainties that still govern our predictions, namely, nuclear yields and heating rates. Our focus will be on the r-process in neutron star (NS) mergers, which is in the spotlight after recent ``multi-messenger'' observations, including the combined detection of gravitational waves from a NS-NS merger event and its subsequent electromagnetic counterpart. In this work, we base our nucleosynthesis calculations on hydrodynamical simulations of NS merger systems, which estimate the amount of ejected mass and its properties during ejection. Through our r-process calculations, we estimate the composition of this gravitationally unbound material, which can contribute to the r-process enrichment of the Galaxy. This work is divided into two studies, each addressing a remaining open question regarding the r-process nucleosynthesis. First, a coherent study of the impact of neutrino interactions on the r-process element nucleosynthesis and the heating rate produced by the radioactive decay of nuclei synthesized in the dynamical ejecta of NS-NS mergers is presented. We have studied the material ejected from four NS-NS merger systems based on hydrodynamical simulations...

==> sections/list_publ.tex <==
%\documentclass[screen,final,english]{../phdulb} 
%\usepackage{../myphdstyle}   % Custom style
%\usepackage{kantlipsum} % Dummy text
%\usepackage{natbib}
%\pagenumbering{gobble}
%\usepackage{epigraph} % for sitater starten ch.
%\usepackage{pdflscape}
%\setsecnumdepth{subsubsection}
%\graphicspath{{../figures/}}
%\usepackage{longtable}
%\begin{document}

\chapter*{List of publications}
\addcontentsline{toc}{chapter}{List of publications}

\begin{enumerate}
\item Goriely, S., Choplin, A., Ryssens, W., \textbf{Kullmann, I.,} \textit{Progress in Nuclear Astrophysics: a multi-disciplinary field with still many open questions}, INPC conference proceeding, submitted

\item Goriely, S. \& \textbf{Kullmann, I.} 2022, \textit{R-process Nucleosynthesis in Neutron-star Merger Ejecta and Nuclear Dependences}, ed. I. Tanihata, H. Toki, \& T. Kajino, \textit{Handbook of Nuclear Physics}, First edition, chapter 5, section 15 (Springer), accepted %\red{DOI}

\item Ryssens, W., Scamps, G., Grams, G., \textbf{Kullmann, I.}, Bender, M., and Goriely, S., \textit{The binding energy of odd-odd nuclei in microscopic mass models}, Journal of Physics: conference series, submitted \\
\url{https://arxiv.org/abs/2211.03667}

\item \textbf{Kullmann, I.}, Goriely, S., Just, O., Bauswein, A., \& Janka, H. T. 2022, \textit{Extensive study of nuclear uncertainties and their impact on the r-process nucleosynthesis in neutron star mergers}, MNRAS submitted \\
\url{https://arxiv.org/abs/2207.07421}

\item Guttormsen, M. Ay, K. O., Ozgur, M., Algin, E., Larsen, A. C., Bello Garrote, F. L., Berg, H. C., Crespo Campo, L., Dahl-Jacobsen, T., Furmyr, F. W., Gjestvang, D., G\"orgen, A., Hagen, T. W., Ingeberg, V. W., Kheswa, B. V., \textbf{Kullmann, I. K. B.}, Klintefjord, M., Markova, M., Midtb\o{}, J. E., Modamio, V., Paulsen, W., Pedersen, L. G., Renstr\o{}m, T., Sahin, E., Siem, S., Tveten, G. M. and Wiedeking, M. 2022, \textit{Evolution of the $\ensuremath{\gamma}$-ray strength function in neodymium isotopes}, Phys. Rev. C, 106, 034314 \\
\url{https://doi.org/10.1103/PhysRevC.106.034314}

\item \textbf{Kullmann, I.}, Goriely, S., Just, O., Ardevol-Pulpillo, R.,  Bauswein, A., Janka, H-T. 2021, \textit{Dynamical ejecta of neutron star mergers with nucleonic weak processes I: Nucleosynthesis}, Monthly Notices of the Royal Astronomical Society, 510, 2804 \\
\url{https://doi.org/10.1093/mnras/stab3393}

\item Just, O., \textbf{Kullmann, I.}, Goriely, S., Bauswein, A., Janka, H-T., Collins, C. E. 2021, \textit{Dynamical ejecta of neutron star mergers with nucleonic weak processes II: Kilonova emission}, Monthly Notices of the Royal Astronomical Society, 510, 2820 \\
\url{https://doi.org/10.1093/mnras/stab3327}

\item \textbf{Kullmann, I. K. B.}, Larsen, A. C., Renstrøm, T., Beckmann, K. S., Bello Garrote, F. L., Crespo Campo, L., Görgen, A., Guttormsen, M., Midtbø, J. E., Sahin, E., Siem, S., Tveten, G. M., Zeiser, F. 2019, \textit{First Experimental Constraint on the $^{191}$Os (n,{$\gamma$}) Reaction Rate Relevant to s-process Nucleosynthesis}, Physical Review C, 99, 065806 \\
\url{https://doi.org/10.1103/PhysRevC.99.065806}
\end{enumerate}

%\end{document}
